Information Security as Strategic (In)effectivity

Security of information flow is commonly understood as preventing any information leakage, regardless of how grave or harmless consequences the leakage can have. In this work, we suggest that information security is not a goal in itself, but rather a means of preventing potential attackers from compromising the correct behavior of the system. To formalize this, we first show how two information flows can be compared by looking at the adversary's ability to harm the system. Then, we propose that the information flow in a system is effectively information-secure if it does not allow for more harm than its idealized variant based on the classical notion of noninterference.

==> subcaption.sty.tex <==
%%
%% This is file `subcaption.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% subcaption.dtx  (with options: `package')
%% 
%% Copyright (C) 1994-2008 Axel Sommerfeldt (caption@sommerfee.de)
%% 
%% --------------------------------------------------------------------------
%% 
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2003/12/01 or later.
%% 
%% This work has the LPPL maintenance status "maintained".
%% 
%% This Current Maintainer of this work is Axel Sommerfeldt.
%% 
%% This work consists of the files caption.ins, caption.dtx, caption2.dtx,
%% ltcaption.dtx, and subcaption.dtx, the derived files caption.sty,
%% caption2.sty, caption3.sty, ltcaption.sty, and subcaption.sty, and the
%% user manuals caption-deu.tex, caption-eng.tex, and caption-rus.tex.
%% 
\NeedsTeXFormat{LaTeX2e}[1994/12/01]
\ProvidesPackage{subcaption}[2008/03/16 v1.0 Adding subcaptions (AR)]
\@ifundefined{caption@subtypehook}{% we need caption v3.1f or newer
  \PackageError{subcaption}{`caption' package not loaded\MessageBreak
    (which is needed by this package)\@gobble}{%
    If you do not understand this error, please take a closer look\MessageBreak
    at the documentation of the `subcaption' package.\MessageBreak
    \@ehc}%
  \endinput}{}
\let\caption@setkeys@ORI\caption@setkeys
\renewcommand\caption@setkeys[2]{\captionsetup[sub]{#2}}
\caption@ExecuteOptions{subcaption}{%
  font+=small,labelformat=parens,labelsep=space,skip=6pt,list=0,hypcap=0}
\caption@ProcessOptions*{subcaption}
\let\caption@setkeys\caption@setkeys@ORI
\let\caption@setkeys@ORI\@undefined
\@ifundefined{c@figure}{}{\DeclareCaptionSubType{figure}}
\@ifundefined{c@table}{}{\DeclareCaptionSubType{table}}
\caption@For{typelist}{\DeclareCaptionSubType{#1}}
\newcommand*\subcaption{\captionsetup{subtype*}\caption}
\g@addto@macro\caption@subtypehook{\let\subcaption\caption}
\caption@For{subtypelist}{%
  \newenvironment{sub#1}%
    {\caption@withoptargs\subcaption@minipage}%
    {\endminipage}}%
\newcommand*\subcaption@minipage[2]{%
  \minipage#1{#2}%
  \captionsetup{subtype}}
\newcommand*\subcaptionbox{\caption@withoptargs\subcaption@box}
\newcommand\subcaption@box[2]{%
  \@testopt{\subcaption@ibox{#1}{#2}}{\wd\@tempboxa}}
\long\def\subcaption@ibox#1#2[#3]{%
  \@testopt{\subcaption@iibox{#1}{#2}{#3}}\subcaptionbox@hj@default}
\long\def\subcaption@iibox#1#2#3[#4]#5{%
  \setbox\@tempboxa\hbox{#5}%
  \begingroup
  \captionsetup{subtype*}% set \caption@position
  \caption@iftop{%
    \endgroup
    \parbox[t]{#3}{%
      \captionsetup{subtype,position=t}%
      \vbox{\caption#1{#2}}%
      \hrule\@height\z@
      \csname caption@hj@#4\endcsname
      \unhbox\@tempboxa}%
  }{%
    \endgroup
    \parbox[b]{#3}{%
      \captionsetup{subtype,position=b}%
      \csname caption@hj@#4\endcsname
      \unhbox\@tempboxa
      \hrule\@height\z@
      \vtop{\caption#1{#2}}}%
  }}
\providecommand*\caption@hj@c{\centering}
\providecommand*\caption@hj@l{\raggedright}
\providecommand*\caption@hj@r{\raggedleft}
\providecommand*\caption@hj@s{}
\newcommand*\subcaptionbox@hj@default{c}
\newcommand*\subfloat{%
  \@ifnextchar[\@subfloat\subfloat@}
\long\def\@subfloat[#1]{%
  \@ifnextchar[{\@@subfloat{#1}}{\subcaptionbox{#1}}}
\long\def\@@subfloat#1[#2]{\subcaptionbox[{#1}]{#2}}
\newcommand*\subfloat@{%
  \caption@teststar\subfloat@@\@firstoftwo\@secondoftwo}
\newcommand\subfloat@@[2]{%
  \setbox\@tempboxa\hbox{#2}%
  \begingroup
  \captionsetup{subtype*}% set \caption@position
  \caption@iftop{\subfloat@@@ t}{\subfloat@@@ b}%
    {#1}\subcaptionbox@hj@default}
\newcommand\subfloat@@@[3]{%
  \endgroup
  \parbox[#1]{\wd\@tempboxa}{%
    #2% \@firstoftwo in star form, \@secondoftwo otherwise
      {\captionsetup{subtype*,position=#1}}%
      {\captionsetup{subtype,position=#1}%
       \caption@refstepcounter\@subcaptype
       \caption@prepareanchor\@subcaptype{}%
       \caption@makeanchor{}}%
    \caption@iftop{\hrule\@height\z@}{}%
    \csname caption@hj@#3\endcsname
    \unhbox\@tempboxa
    \caption@iftop{}{\hrule\@height\z@}}}%
\g@addto@macro\caption@subtypehook{%
  \ifx\label\subcaption@label \else
    \let\subcaption@ORI@label\label
    \let\label\subcaption@label
  \fi}
\newcommand*\subcaption@label[1]{%
  \@bsphack\begingroup
    \subcaption@ORI@label{#1}%
    \protected@edef\@currentlabel{\csname thesub\@captype\endcsname}%
    \subcaption@ORI@label{sub@#1}%
  \endgroup\@esphack}
\DeclareRobustCommand*\subref{\caption@withoptargs\subcaption@ref}
\newcommand*\subcaption@ref[2]{\ref#1{sub@#2}}
\endinput
%%
%% End of file `subcaption.sty'.

